Enhancing RL Safety with Counterfactual LLM Reasoning

Reinforcement learning (RL) policies may exhibit unsafe behavior and are hard to explain. We use counterfactual large language model reasoning to enhance RL policy safety post-training. We show that our approach improves and helps to explain the RL policy safety.

==> old.tex <==
For instance, if it is no longer possible to select all initially available actions, such as due to a defect~\cite{de2021developing,zinn2021fault}, does the trained RL policy still contain knowledge of an alternative plan to fulfill its objective?

In this work, we apply RL policy model checking, which allows us to extract alternative plans to maintain safety properties when specific actions are no longer possible.
This is similar to counterfactual explanations, but instead of being interested in single state-action pairs in the context of accumulated reward, we are interested in alternative policies included inside the trained RL policy that maintain user-specific complex safety properties.


In more detail, our approach takes three inputs: a \emph{Markov Decision Process (MDP)} representing the RL environment, a trained policy, and a PCTL formula for safety measurements.
We \emph{incrementally build} only the reachable parts of the MDP, guided by the trained policy~\cite{DBLP:conf/setta/Gross22}.
We then verify the policy's safety using the Storm model checker~\cite{DBLP:journals/sttt/HenselJKQV22} and the PCTL formula.


We classify two types of action verification: \emph{Alternative Internal Policy Verification}, which involves disabling the first policy choice at each state, taking alternative actions, and comparing the safety measurements to assess the importance of the disabled action (for explaining the inner workings of the trained RL policy); and \emph{Action Redundancy Verification}, which examines if the RL policy maintains performance when specific actions in the entire environment are disabled (for defective controller analysis).

Furthermore, we define \emph{top-k action robustness} concerning a safety property that builds all the possible trajectories inside the MDP for the top-k actions at every state.


Through experiments, we demonstrate the potential of model checking in the context of explainable RL to explain RL policies concerning safety properties.


To summarize, our \textbf{main contribution} demonstrates the advantage of using model checking to enhance explainable RL. 
This approach improves the understandability of RL policies and shows, in addition to its main action selections, what the policy has learned about the underlying environment.


\paragraph{Related Work.}
There exists a variety of related work focusing on the trained RL policy verification~\cite{DBLP:conf/sigcomm/EliyahuKKS21,DBLP:conf/sigcomm/KazakBKS19,pmlr-v161-corsi21a,DBLP:journals/corr/DragerFK0U15,DBLP:conf/pldi/ZhuXMJ19,DBLP:conf/seke/JinWZ22}.

Gross et al. combine verification with explainable RL policy verification in which they present a method that investigates how specific neuron interconnections, specifically input neurons, influence safe decision-making by applying pruning methods on the trained RL policy~\cite{esann2024_gross}.
In comparison, we investigate the actions of the trained RL policy by disabling the RL policy actions and categorize two types of action verification: alternative internal policy and action redundancy verification (see Sectin~\ref{sec:met}).

Our work is, therefore, similar to counterfactual explanations, which are local explanations that analyze what is changed concerning collected accumulated reward if an alternative action is chosen at a state~\cite{DBLP:conf/aaai/Madumal0SV20}.
Unlike counterfactual explanations, we focus on global explanations, such as determining whether a trained RL policy maintains safety if a particular action is no longer allowed.
This is useful for identifying redundant actions~\cite{DBLP:conf/uai/BaramTM21} in the context of safety properties and interpreting whether the policy has enough knowledge of the environment to have an alternative internally encoded.

Baram et al. present algorithms to minimize action redundancy~\cite{DBLP:conf/uai/BaramTM21}.
Zhong et al. examine the theoretical analysis of what action can be eliminated in policy optimization and propose a redundant action filtering mechanism~\cite{DBLP:conf/aaai/ZhongYZ24}.
Our work can also be used to detect redundant actions but within the focus of exact safety property verification.
However, we focus mainly on detecting whether an already trained RL policy can achieve the same safety performance without action as with it by combining model checking with explainable RL.
Our focus is, therefore, on safety and explainable RL rather than RL policy optimization.

Other related works include discretizing continuous actions~\cite{DBLP:conf/icml/DadashiHVGRGP22} and safety shields~\cite{DBLP:conf/aaai/Carr0JT23} that block unsafe actions.

However, we focus on merging model checking of policy safety properties with explainable RL to create explainable and safe RL systems.


\paragraph{Alternative Internal Policy Verification.} The same building procedure is followed, but with a modification: at each state $s$, instead of taking the action $a = \pi(s) = \arg\max_{a \in \text{Act}} f(s)$, we disable this highest-valued action and take the second, third, etc., choices in sequence.
This means that at each state, we evaluate the impact of not selecting the top action by systematically selecting the next best action as determined by the neural network.
We then compare the safety measurement of these alternative DTMCs to the original safety measurement to investigate how essential the initially highest-valued action is for the trained RL policy.

This comparison helps us understand the policy's internal representation of alternative policies to maintain safety.

\paragraph{Action Redundancy Verification.} Another approach to verifying the policy involves investigating whether the RL policy performs as expected when specific actions are disabled across the entire MDP.
This method involves systematically disabling specific actions globally and observing the policy's resulting performance.
By comparing the safety measurements of the DTMCs generated with certain actions disabled to the original DTMC, we can determine if the policy relies heavily on particular actions or if it can still maintain certain safety properties despite their absence.

This analysis helps identify redundant or non-critical actions within the RL policy, providing more insights into its flexibility to maintain safety.

\paragraph{Action Robustness} Furthermore, we allow at each state all top n actions and define action robustness concerning a safety property as the policy property of not violating the user-specified safety property when allowing the one of the top n actions at every state. That means $Pmax-Pmin=0$.

\paragraph{Limitations.} Our method supports memoryless NN policies within modeled MDP environments, only limited by state space and transition count~\cite{DBLP:conf/setta/Gross22}.
